Collaboration Versus Cheating

We outline how we detected programming plagiarism in an introductory online course for a master's of science in computer science program, how we achieved a statistically significant reduction in programming plagiarism by combining a clear explanation of university and class policy on academic honesty reinforced with a short but formal assessment, and how we evaluated plagiarism rates before SIGand after implementing our policy and assessment.

==> acmart-preload-hook.tex <==
% this file is used to pre-load packages before acmart does it wrong...
\PassOptionsToPackage{table,xcdraw,prologue}{xcolor}
%\PassOptionsToPackage{pdflang={en-US}}{hyperref}
